3D-LMVIC: Learning-based Multi-View Image Coding with 3D Gaussian Geometric Priors

Existing multi-view image compression methods often rely on 2D projection-based similarities between views to estimate disparities. While effective for small disparities, such as those in stereo images, these methods struggle with the more complex disparities encountered in wide-baseline multi-camera systems, commonly found in virtual reality and autonomous driving applications. To address this limitation, we propose 3D-LMVIC, a novel learning-based multi-view image compression framework that leverages 3D Gaussian Splatting to derive geometric priors for accurate disparity estimation. Furthermore, we introduce a depth map compression model to minimize geometric redundancy across views, along with a multi-view sequence ordering strategy based on a defined distance measure between views to enhance correlations between adjacent views. Experimental results demonstrate that 3D-LMVIC achieves superior performance compared to both traditional and learning-based methods. Additionally, it significantly improves disparity estimation accuracy over existing two-view approaches.

==> draft.tex <==
Experimental results demonstrate that 3D-GP-LMVIC surpasses both traditional and learning-based methods in performance, while maintaining fast encoding and decoding speed. 

Existing multi-view image compression methods often rely on 2D projection similarities between views to estimate disparity, performing well with small disparities, such as in stereo images, but struggling with more complex disparities from wide-baseline multi-camera systems, common in virtual reality and autonomous driving systems. To overcome this limitation, we propose a novel approach: learning-based multi-view image compression with 3D Gaussian geometric priors (3D-GP-LMVIC) that incorporates 3D Gaussian Splatting to derive geometric priors for accurate disparity estimation. Additionally, we introduce a depth map compression model to reduce redundancy in geometric information across views. A multi-view sequence ordering method is also proposed to enhance correlations between adjacent views. Experimental results show that 3D-GP-LMVIC outperforms both traditional and learning-based methods in overall performance. Additionally, the proposed method demonstrates improved disparity estimation accuracy compared to existing two-view disparity estimation approaches.

% 如图1所示，与以往尝尝关注的立体相机系统不同，3D应用往往通过wide-baseline multi-camera采集场景的全局信息。在这种场景中相机之间的位置与拍摄视角相比于立体相机会有很大差距，这导致了视角之间拍摄的图像会有比较大的视差。现有的视差估计方法往往通过在图像域的邻近位置找寻相似的局部来做视差估计，这种思路在面对复杂的大视差估计时面临挑战。

% 3D Gaussian Splatting介绍，速度，重构质量等。

In addition, we are impressed by 3D Gaussian Splatting (3D-GS) \citep{kerbl20233d}, a novel technique for generating 3D representations from multi-view images and synthesizing novel views. This method achieves remarkable results by representing scenes as mixtures of small, colored Gaussians, capturing intricate geometric details and continuous depth and texture variations. The probabilistic nature of Gaussians allows for smooth, accurate modeling of complex surfaces, enabling the creation of realistic and detailed 3D environments. Additionally, the fast differentiable renderer inherent in 3D Gaussian Splatting ensures efficient real-time inference.

\(\text{aug}\) denotes the operation of augmenting a vector by adding an additional dimension with a value of 1 as its final element. Conversely, \(\text{deaug}\) refers to the operation of reducing a vector by removing its last dimension.

As depicted in \figureautorefname~\ref{fig:ict_module}, the input feature \(\boldsymbol{f}^{i^*}_{n}\) from the backbone network and the aligned feature of \(\boldsymbol{h}^i_{n-1}\) via \(\boldsymbol{\Delta}^i_n\) are concatenated after a convolutional layer. The concatenated feature is then element-wise multiplied with \(\boldsymbol{f}^i_{n,\text{m}}\), followed by a residual block for feature refinement. \textcolor{red}{Multiplication with the feature masks filters relevant information from the reference features.} The final step involves element-wise addition of this refined feature to \(\boldsymbol{f}^{i^*}_{n}\), yielding the output feature \(\boldsymbol{f}^i_{n}\).

% Appendix~\label{appendix:experiment_details}进一步探讨了\eqref{eq:image_mask}中的mask与对齐时产生的鬼影之前的关系。

Appendix~\ref{appendix:visualization}提供了视觉比较的例子。Appendix~\ref{appendix:complexity}提供了计算复杂度分析。Appendix~\ref{appendix:supplementary_coding_performance} provides supplementary experiments on coding performance.

\tableautorefname~\ref{table:complexity} presents Multiply-Accumulate Operations (MACs), model parameters, coding speed, and memory usage of eight learning-based image codecs, evaluated on a platform equipped with an Intel(R) Xeon(R) Gold 6330 CPU @ 2.00GHz and an NVIDIA RTX A6000 GPU.
% a GPU with 10,752 parallel processing cores
The neural network components of the codecs were executed on the GPU, while the entropy coding was handled by the CPU. The open-source code of BiSIC does not provide separate encoder and decoder implementations, so we only measured its overall computational complexity. The computational complexity of the proposed 3D-LMVIC is within an acceptable range, overall comparable to that of the SOTA BiSIC and slightly better than BiSIC-Fast. 3D-LMVIC achieved encoding and decoding times of 0.19s and 0.18s, respectively, making it one of the faster methods. The MACs of the encoder in 3D-LMVIC is relatively large, but it should still be smaller than those of BiSIC. Since BiSIC uses a symmetric encoder-decoder structure, we estimate that the MACs for its encoder and decoder each account for approximately half of the total MACs. Furthermore, in addition to designing an image codec, we also designed a depth map codec, which is another reason for the larger MACs and model parameter count.

\begin{figure*}[thb]
    \centering
    \includegraphics[width=\linewidth]{Figures/3D-GP-LMVIC_pipe_and_illust_of_disp_pred_v2.pdf}
    \vskip -0.1in
    \caption{(a) Overview of the 3D-LMVIC pipeline. (b) Depth-based disparity estimation process.}
    \label{fig:3d-gp-lmvic-pipeline_and_illust_of_disp_est}
    \vskip -0.2in
\end{figure*}
